PMT: Power Measurement Toolkit

Efficient use of energy is essential for today's supercomputing systems, as energy cost is generally a major component of their operational cost. Research into "green computing" is needed to reduce the environmental impact of running these systems. As such, several scientific communities are evaluating the trade-off between time-to-solution and energy-to-solution. While the runtime of an application is typically easy to measure, power consumption is not. Therefore, we present the Power Measurement Toolkit (PMT), a high-level software library capable of collecting power consumption measurements on various hardware. The library provides a standard interface to easily measure the energy use of devices such as CPUs and GPUs in critical application sections.

==> sections/acm-badges.tex <==
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{black},
    keywordstyle=\color{black},
    numberstyle=\tiny\color{black},
    stringstyle=\color{black},
    basicstyle=\small\normalfont\sffamily,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}
\section*{Reproducibility Initiative}
To reproduce our results, you can install PMT yourself and run the benchmarks that we used to demonstrate PMT. In the following subsections, we first list all the relevant software versions, next, we describe how PMT is installed, and we describe how the benchmarks can be executed and how the plots are generated.

\subsection{Software Packages}
Software packages can be installed using Spack \cite{gamblin_todd_2022_6973617}. A recent version of \texttt{git} and \texttt{cmake} are required.
The \texttt{cuda} package is required to use PMT with NVIDIA GPUs. For AMD GPUS, the \texttt{rocm-smi-lib} is needed. Furthermore, the \texttt{hip} package is required to run the provided benchmarks.

We employed the following software versions:

\begin{table}[H]
    \centering
\scalebox{1}{
\begin{tabular}{l|l}
\toprule
\textbf{Software} & \textbf{Version} \\
\midrule
spack & 17.1.0\\ \hline
gcc & 9.4.0\\ \hline
git & 2.31.1\\ \hline
cmake & 3.21.4\\ \hline
cuda & 11.5.0\\ \hline
hip & 4.3.1\\ \hline
python & 3.8.12\\ \hline
py-pybind11 & 2.8.1\\ \hline
rocm-smi-lib & 4.3.1\\
\bottomrule
\end{tabular}
}
\end{table}


\subsection{PMT installation}

Make sure to load the environment modules, such as \texttt{cuda}, or install the packages mentioned above system-wide. Then, download and install the default PMT features such as Rapl.

\begin{lstlisting}[language=bash]
git clone https://git.astron.nl/RD/pmt.git
mkdir build && cd build
cmake .. -DCMAKE_INSTALL_PREFIX=../install
make -j install
\end{lstlisting}

The previous command can be enrich with the features that the user would like to add, e.g. \texttt{-DBUILD\_NVML=ON}.

Otherwise the user can select a custom option such as building NVML or ROCM support by accessing the CMake graphic interface by running (in the build folder):

\begin{lstlisting}[language=bash]
ccmake .
\end{lstlisting}

After selecting the additional features, the library can be rebuilt:
\begin{lstlisting}[language=bash]
make -j install
\end{lstlisting}

\vspace{0.5cm}
Another installation method is using Spack with the custom recipe in \cite{schaap-spack}, which are developed for the Square Kilometre Array (SKA) project by the Schaap Team. After adding the Spack repository to a new Spack environment by using the command:
\begin{lstlisting}[language=bash]
spack repo add schaap-spack
\end{lstlisting}

The PMT package can be just installed by running:

\begin{lstlisting}[language=bash]
spack install pmt
\end{lstlisting}

\subsection{Benchmarks}
If PMT is built from the source code, the PMT install folder should be added to the linker path:

\begin{lstlisting}[language=bash]
export LD_LIBRARY_PATH=$LD_LIBRARY_PATH:<user_path>/pmt/install$
\end{lstlisting}

In case the user would like to use the Python bindings after installing PMT from the source code, the Python library path must be added to the Python path:

\begin{lstlisting}[language=bash]
export PYTHONPATH=PYTHONPATH:<user_path>/pmt/install/lib/python$
\end{lstlisting}

Note that the previous two steps are not required if the user has installed PMT using Spack.

\vspace{0.5cm}

We provide the benchmarks employed at this link \url{https://gitlab.com/p7294/pmt-bench.git}

The benchmarks can be built using CMake. Otherwise, we prepared installation scripts in the \texttt{scripts} folder such as \texttt{install\_nvidia.sh}
Before running building the benchmarks, the user must source the environment variables in the scripts in the \texttt{share} folder by running:

\begin{lstlisting}[language=bash]
source ./share/setup-env.sh
\end{lstlisting}

If the user targets an NVIDIA GPU, additional environmental variables are needed:
\begin{lstlisting}[language=bash]
source ./share/setup-hip-nvidia.sh
\end{lstlisting}

After compiling the benchmark, create a folder called \texttt{res} and run the benchmarks.

\subsection{Plotting the results}

We provide a Jupyter notebook (\url{https://gitlab.com/p7294/pmt-bench.git}, in the \texttt{plot} folder) to plot the results stored in the \texttt{res} folder.
To run the notebook some python packages are required: \texttt{matplotlib}, \texttt{seaborn}, \texttt{pandas}, \texttt{numpy} and \texttt{scipy}.
